Maximizing Coverage Centrality via Network Design: Extended Version

Network centrality plays an important role in many applications. Central nodes in social networks can be influential, driving opinions and spreading news or rumors.In hyperlinked environments, such as the Web, where users navigate via clicks, central content receives high traffic, becoming targets for advertising campaigns. While there is an extensive amount of work on centrality measures and their efficient computation, controlling nodes' centrality via network updates is a more recent and challenging problem. Performing minimal modifications to a network to achieve a desired property falls under the umbrella of network design problems. This paper is focused on improving the coverage centrality of a set of nodes, which is the number of pairs of nodes that have a shortest path passing through the set, by adding edges to the network. We prove strong inapproximability results and propose a greedy algorithm for maximizing coverage centrality. To ensure scalability to large networks, we also design an efficient sampling algorithm for the problem. In addition to providing an extensive empirical evaluation of our algorithms, we also show that, under some realistic constraints, the proposed solutions achieve almost-optimal approximation for coverage centrality maximization.

==> 1_1_application.tex <==
\textbf{Applications:}
In many real life scenarios, increment in coverage of a set of nodes becomes important and we will give a few such examples. 


\textbf{\underline{Application 1 (Better information flow)}:} While information and influence propagation are traditionally modelled as a diffusion process (i.e., using all possible paths)~\cite{kempe2003maximizing}, multiple recent approaches focus on the most probable (shortest) paths in order to allow scalable solutions~\cite{kimura2006tractable,chen2010scalable}.
So, a goal to achieve better information propagation through a set of target nodes of interest, one needs to improve the shortest path based centralities of them. Improving coverage centrality serves the purpose. 

% Linkedin, the social networking site for professionals, always shows the people on the shortest paths between two unconnected persons. Inherently, a person becomes more central just based on its coverage centrality. Increasing coverage centrality increases the possibility of being shown. A company might want to increase coverage centrality of a group of recruiters (target nodes) by connecting to a few people and to be shown more often in these suggestions.


%\textbf{\underline{Application 2 (Airlines network)}:} \todo{need discussion}In booking flights, people are concerned about two things: time and number of hops. The hops are generally the hub airports for the airlines. An airline might be interested in improving the overall hop counts by incrementing the number of flights through a target set of a few airports with good facilities. If having at least one flight represents an edge between two airports, the problem boils down to a coverage centrality optimization problem of these airports as target nodes. The company wants to increase the overall coverage centrality of the target airports by adding a few new flights between them and other airports.


\textbf{\underline{Application 2 (Other metrics)}:} The coverage centrality is a fundamental measure of the network and describes how well positioned the nodes are in the network. Increasing this centrality of a target set of nodes might result in the improvement of various other relevant metrics which have a similar notion of centrality. In Section \ref{sec:exp}, we show that improving coverage centrality leads to more influence spreading capability of the target nodes. It also results in increasing ``closeness" from target to other nodes as well as decreasing the "distances" between the same. Improving these metrics already have very well known applications \cite{Khalil2014, parotsidis2016centrality}. For instance, improving influence maximization of target nodes can improve the content propagation in the network specially when these nodes act as sources. 

\textbf{\underline{Application 3 (Recommendation)}:} In \cite{parotsidis2016centrality}, the authors choose the edges from a pool of recommended ones to decrease the distance from a source to all others. If the edges by our algorithms are chosen among the recommended edges, the coverage of the target nodes will increase and thus they will become more central in the network. 


%\todo{do we need to show experiments for all these applications?}

==> remove_cite.tex <==
%@article{saha2015approximation,
 % title={Approximation algorithms for reducing the spectral radius to control epidemic spread},
  %author={Saha, Sudip and Adiga, Abhijin and Prakash, B Aditya and Vullikanti, Anil Kumar S},
  %journal={arXiv preprint arXiv:1501.06614},
  %year={2015},
  %publisher={SIAM}
%}
@inproceedings{papagelis2011,
 author = {Papagelis, Manos and Bonchi, Francesco and Gionis, Aristides},
 title = {Suggesting Ghost Edges for a Smaller World},
 booktitle = {CIKM},
 pages = {2305--2308},
 year = {2011}
 
} 

@article{o1994hub,
  title={The hub network design problem: a review and synthesis},
  author={O'Kelly, Morton E and Miller, Harvey J},
  journal={Journal of Transport Geography},
  pages = "31--40",
  year={1994}
 
}
